EduNLP: Towards a Unified and Modularized Library for Educational Resources

Educational resource understanding is vital to online learning platforms, which have demonstrated growing applications recently. However, researchers and developers always struggle with using existing general natural language toolkits or domain-specific models. The issue raises a need to develop an effective and easy-to-use one that benefits AI education-related research and applications. To bridge this gap, we present a unified, modularized, and extensive library, EduNLP, focusing on educational resource understanding. In the library, we decouple the whole workflow to four key modules with consistent interfaces including data configuration, processing, model implementation, and model evaluation. We also provide a configurable pipeline to unify the data usage and model usage in standard ways, where users can customize their own needs. For the current version, we primarily provide 10 typical models from four categories, and 5 common downstream-evaluation tasks in the education domain on 8 subjects for users' usage. The project is released at: https://github.com/bigdata-ustc/EduNLP.

==> tables/app_data_downstream.tex <==

\begin{table}[h]
\centering
\caption{Statistics for downstream datasets in Math.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Task} & \textbf{train}    & \textbf{dev} &  \textbf{test} \\
        \hline 
        \textbf{Knowledge}     & 400000 & 83851  & 90722   \\
        \hline 
        \textbf{Difficulty}     & 3600 & 720  & 145   \\
        \hline 
        \textbf{Discrimination}     & 1600 & 400  & 500   \\
        \hline 
        \textbf{Quality}     & 2998 & 790  & 1222   \\
        \hline 
        \textbf{Similarity}     & - & -  & 6873   \\
        \hline
    \end{tabular}
    \label{tab:app_data_downstream}
\end{table}

% \hline 
% midrule 
% toprule
% bottomrule

% \textbf{483851}                & -                       & 90722                                  \\
% \textbf{3600}                  & -                       & \multicolumn{1}{l}{145(from 7 papers)} \\
% \textbf{2000}                  & -                       & 500                                    \\
% \textbf{2998}                  & \multicolumn{1}{r}{790} & 1222                                   \\
% \multicolumn{1}{l}{\textbf{-}} & -                       & 25293  

==> tables/dataset.tex <==
\begin{table}[t]
    \caption{Collected datasets in EduData.\yuting{subject}}
    \centering
    % \begin{tabular}{ccc}
    \begin{tabular}{ccc}
        \toprule
        % \hline
        \textbf{DataSet}    & \textbf{\#Questions} & \textbf{Description}  \\
        \midrule
        % \hhline{-||--}
        % \hline
        OpenEdu9K    & 9000         & -                \\ 
        % \hline
        \midrule
        SVAMP~\cite{SVAMP-patel-etal-2021-nlp}      & 1000           & -                \\
        MaWPS~\cite{MaWPS-koncel-kedziorski-etal-2016-mawps}      & 2373           & -                \\
        math23k~\cite{math23k-wang-etal-2017-deep}    & 23162       & -                \\
        Ape210k~\cite{Ape210k-zhao2020ape210k}    & 210288      & -                \\
        % \hline
        \midrule
        AQUA-RAT~\cite{AQUA-RAT-ling-etal-2017-program}   & 97975          & -                \\ 
        GSM8K~\cite{GSM8K-cobbe2021training}      & 8792           & -                \\ 
        mathQA~\cite{mathQA-amini-etal-2019-mathqa}     & 37200          & -                \\
        % \hline
        \midrule
        Hmwp~\cite{Hmwp-qin-etal-2020-semantically}       & 5491        & -                \\
        Lmwp~\cite{Lmwp-liu-2021-make}       & 5447        & -                \\
        % \midrule
        % Opt     & -          & -                \\
        \bottomrule
        % \hline
    \end{tabular}
    \label{tab:statistics}
\end{table}
